Lorentz and permutation invariants of particles III: constraining non-standard sources of parity violation

Comparisons of the positive and negative halves of the distributions of parity-odd event variables in particle-physics experimental data can provide sensitivity to sources of non-standard parity violation. Such techniques benefit from lacking first-order dependence on simulations or theoretical models, but have hitherto lacked systematic means of enumerating all discoverable signals. To address that issue this paper seeks to construct sets of parity-odd event variables which may be proved to be able to reveal the existence of any Lorentz-invariant source of non-standard parity violation which could be visible in data consisting of groups of real non space-like four-momenta exhibiting certain permutation symmetries.

==> examples/independence/pqabc/collisionEvents/var10.tex <==
% Do not edit
% This LaTeX was generated by
% /Users/lester/LESTERHOME/proj/papers/2018LORENTZ/20200407a-full-S2S30-03.nb
% on Tue 30 Jun 2020 09:44:22
% It contains some momentum values that should zero V1 to V19 with the exception of V10
% A copy of the above workbook may also have been saved as notebook.nb in the current directory.
\gdef\ugrfguijoooopE{\frac{5}{4}}
\gdef\ugrfguijoooopX{0}
\gdef\ugrfguijoooopY{0}
\gdef\ugrfguijoooopZ{1}
\gdef\ugrfguijoooopEdu{\frac{5}{4}}
\gdef\ugrfguijoooopXdu{0}
\gdef\ugrfguijoooopYdu{0}
\gdef\ugrfguijoooopZdu{1}
\gdef\ugrfguijooooqE{2}
\gdef\ugrfguijooooqX{0}
\gdef\ugrfguijooooqY{0}
\gdef\ugrfguijooooqZ{-1}
\gdef\ugrfguijooooqEdu{2}
\gdef\ugrfguijooooqXdu{0}
\gdef\ugrfguijooooqYdu{0}
\gdef\ugrfguijooooqZdu{-1}
\gdef\ugrfguijooooaE{\frac{1}{2} \sqrt{\frac{1}{2} u_{4} \left(\sqrt{u_{4}^2+48}-u_{4}\right)+8}}
\gdef\ugrfguijooooaX{\frac{1}{2} \sqrt{\frac{1}{2} u_{4} \left(\sqrt{u_{4}^2+48}-u_{4}\right)+4}}
\gdef\ugrfguijooooaY{0}
\gdef\ugrfguijooooaZ{0}
\gdef\ugrfguijooooaEdu{\frac{\sqrt{11}}{2}}
\gdef\ugrfguijooooaXdu{\frac{\sqrt{7}}{2}}
\gdef\ugrfguijooooaYdu{0}
\gdef\ugrfguijooooaZdu{0}
\gdef\ugrfguijoooobE{\sqrt{2}}
\gdef\ugrfguijoooobX{\frac{1}{2}}
\gdef\ugrfguijoooobY{\frac{\sqrt{3}}{2}}
\gdef\ugrfguijoooobZ{0}
\gdef\ugrfguijoooobEdu{\sqrt{2}}
\gdef\ugrfguijoooobXdu{\frac{1}{2}}
\gdef\ugrfguijoooobYdu{\frac{\sqrt{3}}{2}}
\gdef\ugrfguijoooobZdu{0}
\gdef\ugrfguijoooocE{\frac{1}{2} \sqrt{\frac{1}{2} u_{4} \left(\sqrt{u_{4}^2+48}-u_{4}\right)+8}}
\gdef\ugrfguijoooocX{-\frac{1}{2} \sqrt{\frac{1}{2} u_{4} \left(\sqrt{u_{4}^2+48}-u_{4}\right)+4}}
\gdef\ugrfguijoooocY{0}
\gdef\ugrfguijoooocZ{0}
\gdef\ugrfguijoooocEdu{\frac{\sqrt{11}}{2}}
\gdef\ugrfguijoooocXdu{-\frac{\sqrt{7}}{2}}
\gdef\ugrfguijoooocYdu{0}
\gdef\ugrfguijoooocZdu{0}


==> examples/independence/pqabc/collisionEvents/var12.tex <==
% Do not edit
% This LaTeX was generated by
% /Users/lester/LESTERHOME/proj/papers/2018LORENTZ/20200407a-full-S2S30-03.nb
% on Tue 30 Jun 2020 09:44:22
% It contains some momentum values that should zero V1 to V19 with the exception of V12
% A copy of the above workbook may also have been saved as notebook.nb in the current directory.
\gdef\ugrfguijoooopE{2}
\gdef\ugrfguijoooopX{0}
\gdef\ugrfguijoooopY{0}
\gdef\ugrfguijoooopZ{1}
\gdef\ugrfguijoooopEdu{2}
\gdef\ugrfguijoooopXdu{0}
\gdef\ugrfguijoooopYdu{0}
\gdef\ugrfguijoooopZdu{1}
\gdef\ugrfguijooooqE{2}
\gdef\ugrfguijooooqX{0}
\gdef\ugrfguijooooqY{0}
\gdef\ugrfguijooooqZ{-1}
\gdef\ugrfguijooooqEdu{2}
\gdef\ugrfguijooooqXdu{0}
\gdef\ugrfguijooooqYdu{0}
\gdef\ugrfguijooooqZdu{-1}
\gdef\ugrfguijooooaE{\sqrt{\frac{3 \left(7+5 \sqrt{2}\right) u_{8}}{2048 u_{7}}+3}}
\gdef\ugrfguijooooaX{1}
\gdef\ugrfguijooooaY{1}
\gdef\ugrfguijooooaZ{\frac{\sqrt{\frac{3}{2} \left(7+5 \sqrt{2}\right)} \sqrt{u_{8}}}{32 \sqrt{u_{7}}}}
\gdef\ugrfguijooooaEdu{\sqrt{3+\frac{3 \left(7+5 \sqrt{2}\right)}{2048}}}
\gdef\ugrfguijooooaXdu{1}
\gdef\ugrfguijooooaYdu{1}
\gdef\ugrfguijooooaZdu{\frac{1}{32} \sqrt{\frac{3}{2} \left(7+5 \sqrt{2}\right)}}
\gdef\ugrfguijoooobE{\sqrt{\frac{3 \left(7+5 \sqrt{2}\right) u_{8}}{2048 u_{7}}+3}}
\gdef\ugrfguijoooobX{\sqrt{2}}
\gdef\ugrfguijoooobY{0}
\gdef\ugrfguijoooobZ{\frac{\sqrt{\frac{3}{2} \left(7+5 \sqrt{2}\right)} \sqrt{u_{8}}}{32 \sqrt{u_{7}}}}
\gdef\ugrfguijoooobEdu{\sqrt{3+\frac{3 \left(7+5 \sqrt{2}\right)}{2048}}}
\gdef\ugrfguijoooobXdu{\sqrt{2}}
\gdef\ugrfguijoooobYdu{0}
\gdef\ugrfguijoooobZdu{\frac{1}{32} \sqrt{\frac{3}{2} \left(7+5 \sqrt{2}\right)}}
\gdef\ugrfguijoooocE{\sqrt{\frac{3 \left(7+5 \sqrt{2}\right) u_{8}}{2048 u_{7}}+6}}
\gdef\ugrfguijoooocX{1}
\gdef\ugrfguijoooocY{-1}
\gdef\ugrfguijoooocZ{\frac{\sqrt{\frac{3}{2} \left(7+5 \sqrt{2}\right)} \sqrt{u_{8}}}{32 \sqrt{u_{7}}}}
\gdef\ugrfguijoooocEdu{\sqrt{6+\frac{3 \left(7+5 \sqrt{2}\right)}{2048}}}
\gdef\ugrfguijoooocXdu{1}
\gdef\ugrfguijoooocYdu{-1}
\gdef\ugrfguijoooocZdu{\frac{1}{32} \sqrt{\frac{3}{2} \left(7+5 \sqrt{2}\right)}}


==> examples/independence/pqabc/collisionEvents/var13.tex <==
% Do not edit
% This LaTeX was generated by
% /Users/lester/LESTERHOME/proj/papers/2018LORENTZ/20200407a-full-S2S30-03.nb
% on Tue 30 Jun 2020 09:44:22
% It contains some momentum values that should zero V1 to V19 with the exception of V13
% A copy of the above workbook may also have been saved as notebook.nb in the current directory.
\gdef\ugrfguijoooopE{2}
\gdef\ugrfguijoooopX{0}
\gdef\ugrfguijoooopY{0}
\gdef\ugrfguijoooopZ{1}
\gdef\ugrfguijoooopEdu{2}
\gdef\ugrfguijoooopXdu{0}
\gdef\ugrfguijoooopYdu{0}
\gdef\ugrfguijoooopZdu{1}
\gdef\ugrfguijooooqE{2}
\gdef\ugrfguijooooqX{0}
\gdef\ugrfguijooooqY{0}
\gdef\ugrfguijooooqZ{-1}
\gdef\ugrfguijooooqEdu{2}
\gdef\ugrfguijooooqXdu{0}
\gdef\ugrfguijooooqYdu{0}
\gdef\ugrfguijooooqZdu{-1}
\gdef\ugrfguijooooaE{\sqrt{\frac{81}{1024 u_{7} u_{8}}+3}}
\gdef\ugrfguijooooaX{1}
\gdef\ugrfguijooooaY{1}
\gdef\ugrfguijooooaZ{\frac{9}{32 \sqrt{u_{7}} \sqrt{u_{8}}}}
\gdef\ugrfguijooooaEdu{\frac{\sqrt{3153}}{32}}
\gdef\ugrfguijooooaXdu{1}
\gdef\ugrfguijooooaYdu{1}
\gdef\ugrfguijooooaZdu{\frac{9}{32}}
\gdef\ugrfguijoooobE{\sqrt{\frac{81}{1024 u_{7} u_{8}}+5}}
\gdef\ugrfguijoooobX{-2}
\gdef\ugrfguijoooobY{0}
\gdef\ugrfguijoooobZ{\frac{9}{32 \sqrt{u_{7}} \sqrt{u_{8}}}}
\gdef\ugrfguijoooobEdu{\frac{\sqrt{5201}}{32}}
\gdef\ugrfguijoooobXdu{-2}
\gdef\ugrfguijoooobYdu{0}
\gdef\ugrfguijoooobZdu{\frac{9}{32}}
\gdef\ugrfguijoooocE{\sqrt{\frac{81}{1024 u_{7} u_{8}}+6}}
\gdef\ugrfguijoooocX{1}
\gdef\ugrfguijoooocY{-1}
\gdef\ugrfguijoooocZ{\frac{9}{32 \sqrt{u_{7}} \sqrt{u_{8}}}}
\gdef\ugrfguijoooocEdu{\frac{5 \sqrt{249}}{32}}
\gdef\ugrfguijoooocXdu{1}
\gdef\ugrfguijoooocYdu{-1}
\gdef\ugrfguijoooocZdu{\frac{9}{32}}


==> examples/independence/pqabc/collisionEvents/var17.tex <==
% Do not edit
% This LaTeX was generated by
% /Users/lester/LESTERHOME/proj/papers/2018LORENTZ/20200407a-full-S2S30-03.nb
% on Tue 30 Jun 2020 09:44:23
% It contains some momentum values that should zero V1 to V19 with the exception of V17
% A copy of the above workbook may also have been saved as notebook.nb in the current directory.
\gdef\ugrfguijoooopE{2}
\gdef\ugrfguijoooopX{0}
\gdef\ugrfguijoooopY{0}
\gdef\ugrfguijoooopZ{1}
\gdef\ugrfguijoooopEdu{2}
\gdef\ugrfguijoooopXdu{0}
\gdef\ugrfguijoooopYdu{0}
\gdef\ugrfguijoooopZdu{1}
\gdef\ugrfguijooooqE{2}
\gdef\ugrfguijooooqX{0}
\gdef\ugrfguijooooqY{0}
\gdef\ugrfguijooooqZ{-1}
\gdef\ugrfguijooooqEdu{2}
\gdef\ugrfguijooooqXdu{0}
\gdef\ugrfguijooooqYdu{0}
\gdef\ugrfguijooooqZdu{-1}
\gdef\ugrfguijooooaE{\sqrt{\frac{81}{1024 u_{12} u_{13}}+5}}
\gdef\ugrfguijooooaX{2}
\gdef\ugrfguijooooaY{0}
\gdef\ugrfguijooooaZ{\frac{9}{32 \sqrt{u_{12}} \sqrt{u_{13}}}}
\gdef\ugrfguijooooaEdu{\frac{\sqrt{5201}}{32}}
\gdef\ugrfguijooooaXdu{2}
\gdef\ugrfguijooooaYdu{0}
\gdef\ugrfguijooooaZdu{\frac{9}{32}}
\gdef\ugrfguijoooobE{\sqrt{\frac{81}{1024 u_{12} u_{13}}+8}}
\gdef\ugrfguijoooobX{-1}
\gdef\ugrfguijoooobY{-\sqrt{3}}
\gdef\ugrfguijoooobZ{\frac{9}{32 \sqrt{u_{12}} \sqrt{u_{13}}}}
\gdef\ugrfguijoooobEdu{\frac{\sqrt{8273}}{32}}
\gdef\ugrfguijoooobXdu{-1}
\gdef\ugrfguijoooobYdu{-\sqrt{3}}
\gdef\ugrfguijoooobZdu{\frac{9}{32}}
\gdef\ugrfguijoooocE{\sqrt{\frac{81}{1024 u_{12} u_{13}}+13}}
\gdef\ugrfguijoooocX{-1}
\gdef\ugrfguijoooocY{\sqrt{3}}
\gdef\ugrfguijoooocZ{\frac{9}{32 \sqrt{u_{12}} \sqrt{u_{13}}}}
\gdef\ugrfguijoooocEdu{\frac{\sqrt{13393}}{32}}
\gdef\ugrfguijoooocXdu{-1}
\gdef\ugrfguijoooocYdu{\sqrt{3}}
\gdef\ugrfguijoooocZdu{\frac{9}{32}}


==> examples/independence/pqabc/collisionEvents/var8.tex <==
% Do not edit
% This LaTeX was generated by
% /Users/lester/LESTERHOME/proj/papers/2018LORENTZ/20200407a-full-S2S30-03.nb
% on Tue 30 Jun 2020 09:44:21
% It contains some momentum values that should zero V1 to V19 with the exception of V8
% A copy of the above workbook may also have been saved as notebook.nb in the current directory.
\gdef\ugrfguijoooopE{1}
\gdef\ugrfguijoooopX{0}
\gdef\ugrfguijoooopY{0}
\gdef\ugrfguijoooopZ{1}
\gdef\ugrfguijoooopEdu{1}
\gdef\ugrfguijoooopXdu{0}
\gdef\ugrfguijoooopYdu{0}
\gdef\ugrfguijoooopZdu{1}
\gdef\ugrfguijooooqE{1}
\gdef\ugrfguijooooqX{0}
\gdef\ugrfguijooooqY{0}
\gdef\ugrfguijooooqZ{-1}
\gdef\ugrfguijooooqEdu{1}
\gdef\ugrfguijooooqXdu{0}
\gdef\ugrfguijooooqYdu{0}
\gdef\ugrfguijooooqZdu{-1}
\gdef\ugrfguijooooaE{\frac{1}{8} \sqrt{\frac{3 u_{1} \left(u_{1}^2-3\right)}{u_{3}-3 u_{1}^2 u_{3}}+64}}
\gdef\ugrfguijooooaX{0}
\gdef\ugrfguijooooaY{0}
\gdef\ugrfguijooooaZ{\frac{i \sqrt{3} \sqrt{u_{1}} \sqrt{u_{1}^2-3}}{8 \sqrt{\left(3 u_{1}^2-1\right) u_{3}}}}
\gdef\ugrfguijooooaEdu{\frac{\sqrt{67}}{8}}
\gdef\ugrfguijooooaXdu{0}
\gdef\ugrfguijooooaYdu{0}
\gdef\ugrfguijooooaZdu{-\frac{\sqrt{3}}{8}}
\gdef\ugrfguijoooobE{\frac{1}{8} \sqrt{\frac{3 u_{1} \left(u_{1}^2-3\right)}{u_{3}-3 u_{1}^2 u_{3}}+320}}
\gdef\ugrfguijoooobX{0}
\gdef\ugrfguijoooobY{2}
\gdef\ugrfguijoooobZ{\frac{i \sqrt{3} \sqrt{u_{1}} \sqrt{u_{1}^2-3}}{8 \sqrt{\left(3 u_{1}^2-1\right) u_{3}}}}
\gdef\ugrfguijoooobEdu{\frac{\sqrt{323}}{8}}
\gdef\ugrfguijoooobXdu{0}
\gdef\ugrfguijoooobYdu{2}
\gdef\ugrfguijoooobZdu{-\frac{\sqrt{3}}{8}}
\gdef\ugrfguijoooocE{\frac{1}{8} \sqrt{\frac{3 u_{1} \left(u_{1}^2-3\right)}{u_{3}-3 u_{1}^2 u_{3}}+128}}
\gdef\ugrfguijoooocX{1}
\gdef\ugrfguijoooocY{0}
\gdef\ugrfguijoooocZ{\frac{i \sqrt{3} \sqrt{u_{1}} \sqrt{u_{1}^2-3}}{8 \sqrt{\left(3 u_{1}^2-1\right) u_{3}}}}
\gdef\ugrfguijoooocEdu{\frac{\sqrt{131}}{8}}
\gdef\ugrfguijoooocXdu{1}
\gdef\ugrfguijoooocYdu{0}
\gdef\ugrfguijoooocZdu{-\frac{\sqrt{3}}{8}}


==> examples/independence/pqabc/collisionEvents/var9.tex <==
% Do not edit
% This LaTeX was generated by
% /Users/lester/LESTERHOME/proj/papers/2018LORENTZ/20200407a-full-S2S30-03.nb
% on Tue 30 Jun 2020 09:44:21
% It contains some momentum values that should zero V1 to V19 with the exception of V9
% A copy of the above workbook may also have been saved as notebook.nb in the current directory.
\gdef\ugrfguijoooopE{1}
\gdef\ugrfguijoooopX{0}
\gdef\ugrfguijoooopY{0}
\gdef\ugrfguijoooopZ{1}
\gdef\ugrfguijoooopEdu{1}
\gdef\ugrfguijoooopXdu{0}
\gdef\ugrfguijoooopYdu{0}
\gdef\ugrfguijoooopZdu{1}
\gdef\ugrfguijooooqE{1}
\gdef\ugrfguijooooqX{0}
\gdef\ugrfguijooooqY{0}
\gdef\ugrfguijooooqZ{-1}
\gdef\ugrfguijooooqEdu{1}
\gdef\ugrfguijooooqXdu{0}
\gdef\ugrfguijooooqYdu{0}
\gdef\ugrfguijooooqZdu{-1}
\gdef\ugrfguijooooaE{\sqrt{\frac{3 \left(1167 u_{1}^2+202\right)}{64 \left(644 u_{1}^3 u_{3}-321 u_{1} u_{3}\right)}+1}}
\gdef\ugrfguijooooaX{0}
\gdef\ugrfguijooooaY{0}
\gdef\ugrfguijooooaZ{\frac{\sqrt{3501 u_{1}^2+606}}{8 \sqrt{u_{1} \left(644 u_{1}^2-321\right) u_{3}}}}
\gdef\ugrfguijooooaEdu{\frac{\sqrt{\frac{24779}{323}}}{8}}
\gdef\ugrfguijooooaXdu{0}
\gdef\ugrfguijooooaYdu{0}
\gdef\ugrfguijooooaZdu{\frac{37 \sqrt{\frac{3}{323}}}{8}}
\gdef\ugrfguijoooobE{\sqrt{\frac{3 \left(1167 u_{1}^2+202\right)}{64 \left(644 u_{1}^3 u_{3}-321 u_{1} u_{3}\right)}+3}}
\gdef\ugrfguijoooobX{-1}
\gdef\ugrfguijoooobY{1}
\gdef\ugrfguijoooobZ{\frac{\sqrt{3501 u_{1}^2+606}}{8 \sqrt{u_{1} \left(644 u_{1}^2-321\right) u_{3}}}}
\gdef\ugrfguijoooobEdu{\frac{3 \sqrt{\frac{7347}{323}}}{8}}
\gdef\ugrfguijoooobXdu{-1}
\gdef\ugrfguijoooobYdu{1}
\gdef\ugrfguijoooobZdu{\frac{37 \sqrt{\frac{3}{323}}}{8}}
\gdef\ugrfguijoooocE{\sqrt{\frac{3 \left(1167 u_{1}^2+202\right)}{64 \left(644 u_{1}^3 u_{3}-321 u_{1} u_{3}\right)}+102}}
\gdef\ugrfguijoooocX{10}
\gdef\ugrfguijoooocY{1}
\gdef\ugrfguijoooocZ{\frac{\sqrt{3501 u_{1}^2+606}}{8 \sqrt{u_{1} \left(644 u_{1}^2-321\right) u_{3}}}}
\gdef\ugrfguijoooocEdu{\frac{3 \sqrt{\frac{234739}{323}}}{8}}
\gdef\ugrfguijoooocXdu{10}
\gdef\ugrfguijoooocYdu{1}
\gdef\ugrfguijoooocZdu{\frac{37 \sqrt{\frac{3}{323}}}{8}}

